Near-the-Axis Universality in Last Passage Percolation

This note establishes a universal directed landscape limit for last passage percolation models in an intermediate scaling regime. We find as a quick consequence the transversal fluctuations for geodesics taken near the axis. We extend the technique of Bodineau and Martin, who in arXiv:math/0410042 have already shown universal one-point fluctuations in this regime.

==> preamble.tex <==
% Updated 2025-08-15
\usepackage{xcolor}
\usepackage[dvipsnames]{xcolor}
\RequirePackage[l2tabu,orthodox]{nag}  % force newer (and safer) LaTeX commands
\RequirePackage[utf8]{inputenc}

\RequirePackage[a4paper]{geometry}
\RequirePackage{microtype}

\RequirePackage{caption, subcaption}

\RequirePackage{mathtools, amssymb, amsthm, thmtools}

\RequirePackage{booktabs, array}

\RequirePackage{appendix}

\RequirePackage{datetime}
\newdateformat{usvardate}{%
	\THEDAY\  \monthname[\THEMONTH] \THEYEAR}
\usvardate


% Fonts
\RequirePackage{amsfonts, mathrsfs, bbm, soul}

\RequirePackage{enumitem}

\RequirePackage{color}

% tikz
% \RequirePackage{tikz}
% \usetikzlibrary {positioning} 
% \usetikzlibrary{arrows.meta}
%\usetikzlibrary{calc,intersections}

% Bibliography
\RequirePackage[backend=biber,style=alphabetic]{biblatex}
\bibliography{biblio.bib}

% Auxiliary commands
\RequirePackage{xspace}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}

% Operators. Usage: \GL
\def\oper#1{\csdmat{#1}{\operatorname{#1}}}
\forcsvlist\oper{GL,SL,deg,Spec,Hom,End,Vect,Mod,Rep,Ker,Im,Id,Aut,lcm, dist, diam, tr, ker, im, Sym, Span, Res, sinc, supp, Arg, var}
\DeclareMathOperator{\RE}{Re}
\DeclareMathOperator{\IM}{Im}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}

% Mathbb Letters. Usage: \bA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\forcsvlist\defbb{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Structures
\def\eq#1{\begin{equation}#1\end{equation}}
\def\ov#1#2{{\substack{#1\\#2}}} % #1 over #2

\def\conj#1{\overline{#1}}
\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}}
\newcommand{\mpder}[3][]{\frac{\partial^{#3}#1}{\partial#2^{#3}}}

% Delimiters
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}
\DeclarePairedDelimiter\brac{\lparen}{\rparen}
\DeclarePairedDelimiter\sqrbrac{[}{]}
\DeclarePairedDelimiter\inner{\langle}{\rangle}
\DeclarePairedDelimiter\set{\{}{\}}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}

% Extended delimiters
\DeclarePairedDelimiterXPP\Ex[1]{\mathbb{E}}[]{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Exsub[2]{\mathbb{E}_{#2}}[]{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Exabs[1]{\mathbb{E}}\lvert\rvert{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Prob[1]{\mathbb{P}}(){}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Probsub[2]{\mathbb{P}_{#2}}(){}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Var[1]{\mathrm{Var}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Cov[1]{\mathrm{Cov}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}
\DeclarePairedDelimiterXPP\Corr[1]{\mathrm{Corr}}\lparen\rparen{}{
\renewcommand\given{\nonscript\:\delimsize\vert\nonscript\:\mathopen{}}
#1}

% Distributions
\newcommand{\Exp}{\ensuremath{\mathrm{Exp}}}
\newcommand{\Ber}{\ensuremath{\mathrm{Ber}}}
\newcommand{\Geom}{\ensuremath{\mathrm{Geom}}}
\newcommand{\Unif}{\ensuremath{\mathrm{Unif}}}

% Shorthands
\newcommand{\disteq}{\ensuremath{\stackrel{d}{=}}}
\newcommand{\distto}{\ensuremath{\stackrel{d}{\to}}}
\newcommand{\given}{\ensuremath{\mid}}
\newcommand{\mto}{\ensuremath{\mapsto}}
\newcommand{\bone}{\mathbbm{1}}

% Wide accents
\DeclareFontFamily{U}{mathx}{}
\DeclareFontShape{U}{mathx}{m}{n}{<-> mathx10}{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareMathAccent{\widehat}{0}{mathx}{"70}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}

% Independece symbols
\RequirePackage{rotating,centernot,cancel}    %% to manipulate symbols 
\def\indep{\ \ \;{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\models$\end{rotate}}}}\ \, }  %independent random variables 
\def\nindep{\ \ \,{\raisebox{-1.5pt}{\text{\begin{rotate}{90}$\nvDash$\end{rotate}}}}\ \, }   %not independent random variables 

% Bolded item numbers
\newcommand{\bitem}[1]{\item[\textbf{#1.}]}

% Mathbb Letters. Usage: \bA
\def\defbb#1{\csdmat{b#1}{\mathbb{#1}}}
\forcsvlist\defbb{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Mathcal Letters. Usage: \cA
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\forcsvlist\defcal{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

% Script Letters. Usage: \sA
\def\defscr#1{\csdmat{scr#1}{\mathscr{#1}}}
\forcsvlist\defscr{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z,a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

% Fraktur Letters. Usage: \frakA
\def\deffrak#1{\csdmat{frak#1}{\mathfrak{#1}}}
\forcsvlist\deffrak{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z,a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}

% Almost everywhere abbreviations
\newcommand{\es}{\ensuremath{\ \mathrm{a.s}}}
\newcommand{\as}{\ensuremath{\ \mathrm{a.s}}}
\newcommand{\io}{\ensuremath{\ \mathrm{i.o}}}
\newcommand{\fo}{\ensuremath{\ \mathrm{f.o}}}

% Macro for nicer restriction spacing

\newcommand{\littletaller}{\mathchoice{\vphantom{\big|}}{}{}{}}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \littletaller % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\RequirePackage[colorlinks,urlcolor=blue,linkcolor=red,citecolor=green, hypertexnames=false]{hyperref}
\RequirePackage[capitalize]{cleveref}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{claim}{Claim}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{remark}[theorem]{Remark}
\def\samnote#1{{\color{blue}{(Sam: #1)}}}
\def\saranote#1{{\color{red}{(Sara: #1)}}}
% Lists inside theorems (for cleverref)
\newlist{thmlist}{enumerate}{1}
\setlist[thmlist]{label=(\roman{thmlisti}), ref=\thetheorem.(\roman{thmlisti})}
\crefname{thmlisti}{theorem}{theorems}
\crefname{proplisti}{proposition}{propositions}

\newlist{proplist}{enumerate}{1}
\setlist[proplist]{label=(\roman{proplisti}), ref=\thetheorem.(\roman{proplisti})}
\crefname{prop}{proposition}{propositions}

\newlist{corlist}{enumerate}{1}
\setlist[corlist]{label=(\roman{corlisti}), ref=\thetheorem.(\roman{corlisti})}
\crefname{cor}{corollary}{Corollaries}

\Crefname{thm}{Theorem}{Theorems}
\Crefname{lem}{Lemma}{Lemmas}
\Crefname{app}{Appendix}{Appendices}
\Crefname{prop}{Proposition}{Propositions}
